Gender Bias in Neural Natural Language Processing

We examine whether neural natural language processing (NLP) systems reflect historical biases in training data. We define a general benchmark to quantify gender bias in a variety of neural NLP tasks. Our empirical evaluation with state-of-the-art neural coreference resolution and textbook RNN-based language models trained on benchmark datasets finds significant gender bias in how models view occupations. We then mitigate bias with CDA: a generic methodology for corpus augmentation via causal interventions that breaks associations between gendered and gender-neutral words. We empirically show that CDA effectively decreases gender bias while preserving accuracy. We also explore the space of mitigation strategies with CDA, a prior approach to word embedding debiasing (WED), and their compositions. We show that CDA outperforms WED, drastically so when word embeddings are trained. For pre-trained embeddings, the two methods can be effectively composed. We also find that as training proceeds on the original data set with gradient descent the gender bias grows as the loss reduces, indicating that the optimization encourages bias; CDA mitigates this behavior.

==> Makefile <==
OS   := $(shell uname)
ifeq ($(OS), Linux)
  OPEN := evince
else
ifneq ("$(wildcard /Applications/Skim.app)","")
  OPEN := open -a /Applications/Skim.app
else
  OPEN := open -a /Applications/Preview.app
endif
endif
DOC  := doc-bias-nlp
MAIN := preamble
PDFLATEX := pdflatex

DEP_FIGS := $(shell find ./figures \
	-name '*.tex' \
	)
DEP := *.tex *.bib $(DEP_FIGS)
DEP := $(foreach i,$(DEP),$(shell ls $(i) 2> /dev/null))

start:
	make draft

start-%:
	make open-$*
	make watch-$*

draft:
	make start-draft

final:
	make start-final

$(DOC).final.main.pdf: $(DOC).final.pdf
	pdftk $(DOC).final.pdf cat 1-9 output $@

$(DOC).final.supplemental.pdf: $(DOC).final.pdf
	pdftk $(DOC).final.pdf cat 10-12 output $@

parts: $(DOC).final.main.pdf $(DOC).final.supplemental.pdf

startt:
	$(PDFLATEX) $(QUIET) preamble; $(BIBTEX) $(QUIET) $(MAIN); $(PDFLATEX) $(QUIET) preamble; $(PDFLATEX) $(QUIET) preamble;
	make clean; $(OPEN) preamble.pdf

open-%: $(DOC).%.pdf
ifneq ("$(OPEN)","")
	$(OPEN) $(DOC).$*.pdf ; sleep 1
else
	@echo "Could not find a PDF reader. If you'd like this \
	makefile to open the generated pdfs, add your PDF reader to \
	the opening section of the Makefile."
	@exit 1
endif

$(DOC).pdf: $(DEP)
	perl watch.pl render_latex $(MAIN) "\input{$(MAIN).tex}"
	@cp $(MAIN).pdf $(DOC).pdf
	@cp $(MAIN).synctex.gz $(DOC).synctex.gz


$(DOC).%.pdf: $(DEP)
	perl watch.pl render_latex $(MAIN) "\def\$*{}\input{$(MAIN).tex}"
	@cp $(MAIN).pdf $(DOC).$*.pdf
	@cp $(MAIN).synctex.gz $(DOC).$*.synctex.gz

watch-%:
	perl watch.pl watch $(DOC).$*.pdf $(DEP)
	perl watch.pl watch $(DOC).pdf $(DEP)

# DEBUGGING UTILS
# https://www.cmcrossroads.com/article/printing-value-makefile-variable
print-%  : ; @echo $* = $($*)

debug: $(DEP)
	$(PDFLATEX) -interaction nonstopmode "\input{$(MAIN).tex}"
	$(OPEN) $(DOC).pdf

# To debug unicode issues:
# useful emacs command: find-file-literally
show_unicode: $(DEP)
	pcregrep --color='auto' -n "[\x80-\xFF]" *.tex *.bib

# List all references to the thing after find_ in the tex sources.
find_%: *.tex
	grep -I -C 1 -n --color=auto '$*' *.tex; true

# CLEANING
clean:
	rm -Rf *.aux *.lof *.log *.lot *.bbl *.blg *.toc *.out *.bcf *.run.xml; true
	rm -Rf *~; true
	rm -Rf $(DOC).pdf $(MAIN).pdf $(DOC).*.pdf; true
	rm -Rf main-blx.bib
	rm -Rf .DS_Store; true
	rm -Rf .iTeXMac; true
	rm -Rf *.*.gz; true
	rm -Rf *.pdfsync; true
	rm -Rf *.synctex; true

desvn:
	find . -type d -name .svn -exec rm -rf {} +

#ARTIFACTS := $(shell find artifact)

#artifact: ${ARTIFACTS}
#	COPYFILE_DISABLE=1 tar -cvf artifact.tar artifact
#	gzip artifact.tar

# PACKAGING

DEP_TEX := $(shell find . \
	-not \( -path ./old-sections -prune \) \
	-not \( -path ./supplemental -prune \) \
	-not \( -path ./ijcai2018-formatting-guidelines -prune \) \
	-not \( -path ./arXiv -prune \) \
	-not \( -path ./formatting_instructions -prune \) \
	-not \( -path ./styles -prune \) \
	-name '*.tex' \
	)

DEP_TEX2 := $(DEP_TEX:%=arXiv/%)

arXiv/%.tex: %.tex
	latexpand --empty-comments $< > arXiv/$<
	sed -e '/^\s*%/d' -i '' arXiv/$<

arXiv:
	mkdir arXiv
	mkdir arXiv/figures

$(MAIN).bbl: $(DOC).arXiv.pdf

bundle: $(MAIN).bbl arXiv $(DEP_TEX:%=arXiv/%) nips_2018.sty
	cp -R $(MAIN).bbl nips_2018.sty arXiv
	cp -R $(DEP_FIGS) arXiv/figures
	(echo "\def\\\\arXiv{}\n"; cat arXiv/$(MAIN).tex) \
           > arXiv/$(MAIN).tex.temp
	mv arXiv/$(MAIN).tex.temp arXiv/$(MAIN).tex
	tar -cvf arXiv.tar arXiv
	gzip arXiv.tar

rebundle:
	rm -Rf arXiv; true
	rm -Rf arXiv.tar.gz; true
	make bundle


==> figures/coref_model.tex <==
\begin{tikzpicture}
  \tikzstyle{every node}=[font=\small,align=center,text width=0.9in, outer sep=4pt]
  \tikzstyle{pointer}=[->,thick]
  \tikzstyle{roundbox}=[draw, rounded corners]

  \node[] (mention) at (-1.25,0)
    {words in \\mention $m: m_i$\\(\emph{he})};

  \node[] (antecedent) at (-1.25,-1.5)
    {words in \\mention $c: c_i$\\(\emph{The}, \emph{doctor})};

  \node[] (metadata) at (-1.25,-3)
    {metadata};

  \node[roundbox] (mentionembeddings) at (3,0)
    {word embeddings \\ of $m_i$};

  \node[roundbox] (antecedentembeddings) at (3,-1.5)
    {word embeddings \\ of $c_i$};

  \node[roundbox] (pairfeatures) at (3,-2.70)
    {pair features};

  \node[] (otherfeatures) at (3,-3.30)
    {other features};

  \node[text width=0.5in] (network) at (6.5,-1.5)
    {feed\\forward\\network};

  \node[roundbox,fit=(otherfeatures)(pairfeatures)] (metadatapart) {};
  \node[roundbox,fit=(mentionembeddings)(otherfeatures)(metadatapart)] (inputspart) {};

  \node[roundbox,fit=(network)(mentionembeddings.north -| network)(metadatapart.south -| network)] (networkbox) {};

  \node[text width=0.5in] (score) at (9.75,-1.5)
    {score\\$\score{m}{c}$};

  \node[inner sep=5pt,roundbox,fit=(otherfeatures)(mentionembeddings)(inputspart)(networkbox)] (allpart) {};

  \path[pointer] (mention) edge (mention -| allpart.west);
  \path[pointer] (antecedent) edge (antecedent -| allpart.west);
  \path[pointer] (metadata) edge (metadata -| allpart.west);
  \path[pointer] (inputspart.east |- score) edge (networkbox.west |- score);
  \path[pointer] (allpart.east |- score.west) edge (score);

\end{tikzpicture}


==> figures/coref_model_simple.tex <==
\begin{tikzpicture}
  \tikzstyle{every node}=[font=\small,align=center,text width=1.0in, outer sep=4pt]
  \tikzstyle{pointer}=[->,thick]
  \tikzstyle{roundbox}=[draw, rounded corners]

  \node[text width=1.0in] (input_document) at (0,0.75)
  {\textbf{text}\\\emph{...\\
      The doctor ran because he$_1$ is late. \\
      ... \\
      The nurse ran because he$_2$ is late. \\
      ...}};

  \node[text width=1in,below=0.25in of input_document] (input_metadata)
    {\textbf{metadata}\\speaker,\\genre,\\...};

  \node[roundbox,text width=0.6in, right=0.25in of input_document] (embedding)
    {\textbf{embedding}\\$\embedding$};



  \node[roundbox,text width=0.5in] at (embedding |- input_metadata) (network)
    {\textbf{feed forward network\\$ffn_\beta$}};

%  \node[roundbox,text width=0.6in,above=0in of network] (features) {\textbf{feature\\constructor}}; 

  \node[roundbox,fit=(network)] (ranker) {};

  \node[text width=1.4in, right=0.25in of network] (scores)
    {\textbf{scores}\\
      $\scoring{The doctor}{he$_1$}{5.56}$\\
      $\scoring{The nurse}{he$_2$}{0.44}$\\
      $\cdots$};

  \node[roundbox,text width=0.5in] at (embedding -| scores) (clusterer) {\textbf{clusterer}};

  \node[right=0.25in of clusterer] (output)
  {\textbf{output}\\\{The doctor, he$_1$\},\\\{The nurse\}, \{he$_2$\},\\...};

  \node[roundbox,below=0.25in of scores] (lossfunc) {\textbf{loss function}\\$L$};

  \node[text width=1.5in] at (input_metadata |- lossfunc) (truth)
  {\textbf{ground truth}\\
    $\set{\text{The doctor}, \text{he}_1}, $\\
    $\set{\text{The nurse}}, \set{\text{he}_2}, $ \\
    $\cdots$};

  \node[text width=0.2in] at (output |- lossfunc) (loss)
  {\textbf{loss}};%\\$\frac{1}{n}L(4.56, 1.0)+$\\$\frac{1}{n}L(0.44, 0.0)$\\...};

  \path[pointer] (input_document) edge (embedding);
  \path[pointer] (input_document) edge (ranker);
  \path[pointer] (embedding) edge (ranker);
  \path[pointer] (input_metadata) edge (ranker);
  \path[pointer] (ranker) edge (scores);
  \path[pointer] (scores) edge (clusterer);
  \path[pointer] (clusterer) edge (output);

%  \path[pointer] (features) edge (network);

  \path[pointer] (truth) edge (lossfunc);
  \path[pointer] (scores) edge (lossfunc);

  \path[pointer] (lossfunc) edge (loss);
 
%  \node[roundbox, inner sep=-1pt, fit=(embedding)(scores),black!50] (system) {};
%  \node[roundbox,fit=(mentionembeddings)(otherfeatures)(metadatapart)] (inputspart) {};
%
%%  \node[roundbox,fit=(network)(mentionembeddings.north -| network)(metadatapart.south -| network)] (networkbox) {};
%
%  \node[text width=0.5in] (score) at (9.75,-1.5)
%    {score\\$s(m,c)$};
%
%%  \node[inner sep=5pt,roundbox,fit=(otherfeatures)(mentionembeddings)(inputspart)(networkbox)] (allpart) {};
%

\end{tikzpicture}


==> figures/retrain.tex <==
\begin{tikzpicture}
  \tikzstyle{every node}=[font=\small,text width=0.5in, outer sep=4pt]
  \tikzstyle{pointer}=[->,thick]
  \tikzstyle{roundbox}=[draw, rounded corners, inner sep=4pt, minimum height=0.4in]
  \tikzstyle{bigroundbox}=[roundbox, text width=2.5in]

  \node[bigroundbox] (original) at (0,0)
    {Original Corpus
    \begin{enumerate}
    \item{} \textbf{The doctor} ate because \textbf{he} is hungry.\\
            (cluster label: [\emph{The doctor}, \emph{he}])
    \item{} \textbf{The nurse} ate because \textbf{she} is hungry.\\
            (cluster label: [\emph{The nurse}, \emph{she}])
    \end{enumerate}
    };

  \node[bigroundbox] (counter) at (0,-2.5)
    {Labeled Counterfactuals
    \begin{enumerate}
    \item{} \textbf{The doctor} ate because \textbf{she} is hungry.\\
            (cluster label: [\emph{The doctor}, \emph{she}])
    \item{} \textbf{The nurse} ate because \textbf{he} is hungry.\\
            (cluster label: [\emph{The nurse}, \emph{he}])
    \end{enumerate}
    };

  \node[roundbox,align=center] (ffn1) at (5,-0.5) {FFN};
  \node[roundbox,align=center] (ffn2) at (5,-2.0) {FFN};
  \node[roundbox,align=center] (omodel) at (7.5,-0.5) {Original\\model};
  \node[roundbox,align=center] (bmodel) at (7.5,-2.0) {Boosted\\model};

  \path[pointer] (original.east |- ffn1) edge (ffn1);
  \path[pointer] (original.-15) edge (ffn2.160);
  \path[pointer] (counter.east |- ffn2)  edge (ffn2);

  \path[pointer] (ffn1) edge (omodel);
  \path[pointer] (ffn2) edge (bmodel);

\end{tikzpicture}

